Automatic Detection and Analysis of Technical Debts in Peer-Review Documentation of R Packages

Technical debt (TD) is a metaphor for code-related problems that arise as a result of prioritizing speedy delivery over perfect code. Given that the reduction of TDs can have long-term positive impact in the software engineering life-cycle (SDLC), TDs are studied extensively in the literature. However, very few of the existing research focused on the technical debts of R programming language despite its popularity and usage. Recent research by Codabux et al. [21] finds that R packages can have 10 diverse TD types analyzing peer-review documentation. However, the findings are based on the manual analysis of a small sample of R package review comments. In this paper, we develop a suite of Machine Learning (ML) classifiers to detect the 10 TDs automatically. The best performing classifier is based on the deep ML model BERT, which achieves F1-scores of 0.71 - 0.91. We then apply the trained BERT models on all available peer-review issue comments from two platforms, rOpenSci and BioConductor (13.5K review comments coming from a total of 1297 R packages). We conduct an empirical study on the prevalence and evolution of 10 TDs in the two R platforms. We discovered documentation debt is the most prevalent among all types of TD, and it is also expanding rapidly. We also find that R packages of generic platform (i.e. rOpenSci) are more prone to TD compared to domain-specific platform (i.e. BioConductor). Our empirical study findings can guide future improvements opportunities in R package documentation. Our ML models can be used to automatically monitor the prevalence and evolution of TDs in R package documentation.

==> automatic-detection.tex <==
\section{RQ1: Automatic Detection of TD}
\subsection{Discarding Insignificant Sentences}
describe stage-1
\subsection{Detection of TD-type}
describe stage-2

==> backup/study_result_backup.tex <==
\section{Automatic Detection of The Smells}
We answer the following four research questions:

\begin{enumerate}[label=RQ\arabic{*}., leftmargin=25pt]
  \item How accurate are rule-based classifiers to automatically detect the documentation smells?
  \item Can the shallow machine learning models outperform the rule-based classifiers?
  \item Can the deep machine learning models outperform the shallow learning models?
  \item Can the detection of one documentation smell support the detection another smell?
\end{enumerate}
\subsection{Performance Metrics}
We analyze and report the performance of each of the techniques developed and experimented as part of the algorithms development steps. We used 5-fold iterative stratified cross-validation for reporting performances that has been recommended for a multilabel dataset in \cite{iterative_stratified_cross_valid}. We report the performances using standard multi-label classification metrics, i.e., Exact Match Ratio, Hamming Loss \cite{a_literature_survey_on_algorithms_for_multilabel}. We also report separate Accuracy, Precision, Recall, and F1-score for each class.

\begin{inparaenum}[(a)]
\item\bf{Iterative Stratified Cross-Validation}
Traditional $k$-fold cross-validation is a statistical method of evaluating machine learning algorithms which divides data into $k$ equally sized folds and runs for $k$ iterations \cite{traditional_cross_validation_paper}. In each iteration, each of the $k$ folds is used as the held-out set for validation while the remaining $k-1$ folds are used as training sets. Stratified cross-validation is used to make sure that each fold is an appropriate representative of the original data by producing folds where the proportion of different classes is maintained \cite{stratified_cross_validation_paper}. However, stratification is not sufficient for multi-label classification problems as the number of distinct labelsets (i.e., different combinations of labels) is often quite large. For example, there can be 32 combinations of labels in our study as there are 5 types of documentation smells. In such cases, original stratified $k$-fold cross-validation is impractical since most groups might consist of just a single example. Iterative stratification, proposed by \cite{iterative_stratified_cross_valid}, solves this issue by employing a greedy approach of selecting the rarest groups first and adding them to the smallest folds while splitting. Hence, we used this iterative stratified cross-validation in our experiment. 

\item\bf{Exact Match Ratio}
In multi-label classification, prediction for an instance is a set of labels. Hence, it has a notion of partially correct prediction (along with fully correct and incorrect). The Exact Match Ratio ($EMR$) ignores the partially correct prediction and considers only those predictions as correct which exactly match the true label sets.

\begin{equation}
EMR  = \frac{1}{N} \sum_{i=1}^{N} I (L_i^{pred} = L_i^{true})
\label{eq:EMR}
\end{equation} %&

{$I$ is the indicator function. Its' value is 1 if the prediction, $L_i^{pred}$ matches the actual label, $L_i^{true}$, and 0 otherwise. $N$ is the total number of data.
}


\item\bf{Hamming Loss}
Hamming Loss ($HL$) is the fraction of labels in labelsets that are incorrectly predicted, i.e., the fraction of the wrong labels to the total number of labels \cite{hamming_loss_paper}. It takes the notion of partially correct prediction into account.  
\begin{equation}
HL  = \frac{1}{N\cdot L} \sum_{i=1}^{N} \sum_{j=1}^{L} xor (y_{i,j}^{pred}, y_{i,j}^{true}) \label{eq:HL}
\end{equation}

{$N$ is the total number of data, $L$ is the total number of labels.}

\item\bf{Accuracy}
Accuracy ($A$) is the number of correctly predicted instances out of all the instances. We reported accuracy separately for each class.
\begin{equation}
A = \frac{TP+TN}{TP+FN+TN+FP}
\label{eq:acc}
\end{equation}

{$TP$ is the number of true positives, $FN$ is the number of false
negatives, $FP$ is the number of false positives, $TN$ is the number of true
negatives.}


\item\bf{Precision}
Precision ($P$) is the ratio between the number of correctly predicted instances and all the predicted instances for a given class.
\begin{equation}
P  = \frac{TP}{TP+FP} 
\label{eq:precision}
\end{equation} %&


\item\bf{Recall}
Recall ($R$) represents the ratio of the number of correctly predicted instances and all instances belonging to a given class.

\begin{equation}
 R = \frac{TP}{TP+FN}
 \label{eq:recall}
 \end{equation} 
 

\item\bf{F1-score}
F1-score is the harmonic mean of precision and recall.
\begin{equation}
F1 = \frac{2\cdot P\cdot R}{P+R}
\label{eq:f-score}    
\end{equation}

\end{inparaenum}

\subsection{ How accurate are rule-based classifiers to automatically detect the documentation smells? (RQ1)}
\subsubsection{Rule-based Metrics}
%\subsubsection{Approach}
%\gias{discuss the studied features, put the feature summaries in a table}
%discuss the features, group the features into a set of feature dimensions.


\begin{inparaenum}[(a)]
\item\bf{Documentation Length.} We use the length of every documentation in order to capture the extensiveness of the bloated documentations.

\item\bf{Readability Metrics.} We measure Flesch readability metrics for the documentations and use them as a feature to analyze the understandability of documentation. This feature might be useful to detect tangled documentations.

\item\bf{Number of Acronyms and Jargons.} Since acronyms and jargons increase the complexity of a reading passage, we use the number of acronyms and jargon in every documentation to detect the tangled documentation by estimating the understandability.

\item\bf{Number of URLs.} As URLs are hints of possible fragmentations in the documentation, we use the number of URLs to capture these smells.

\item\bf{Number of function, class and package name mentioned.} We use the number of functions, classes, packages mentioned in documentation to capture excess structural information and fragmentation.

\item\bf{Edit Distance.} From the definition of lazy documentation, it can be said that the edit distance of a lazy documentation and its’ unit definition (method prototype) will be comparatively small. So we calculate the edit distance between the documentation description and method prototype and use it as a feature for our machine learning models.

\item\bf{Average Cosine Similarity.} We calculate the avg. cosine similarity of the documentations’ description. For this, we calculate the cosine similarities between each possible pair of that documentation and take their avg value for normalization. This feature will help to detect redundancy in the documentations.
\end{inparaenum}

\subsubsection{Results}
discuss the results by varying the metric thresholds

\subsection{How accurate are shallow machine learning models to automatically detect the documentation smells? (RQ2)}
\subsubsection{Shallow Learning Models}
We applied both traditional and deep learning algorithms to detect documentation smells. We employed different decomposition approaches (i.e., One-Vs-Rest, Label Powerset, Classifier Chains)~\cite{multilabel_decomp_1_MultilabelClassificationAnOverview,multilabel_decomp_2_AReviewOnMultilabelLearning,multilabel_decomp_3_ATutorialOnMultilabelClassification,multilabel_decomp_4_LearningFromMultilabelData} with Support Vector Machine (SVM) \cite{SVM_SupportVectorNetworks} as the base estimator for multi-label classification of documentation smells. We chose SVM since it has been successfully used with these decomposition approaches for multi-label classification in previous studies \cite{SVM_multi_1_AKernelMethodForMultilabelled, SVM_multi_2_TextCategorizationWithSVM}. SVM has also shown great performance in text classification tasks \cite{svm_text_classification_1, svm_text_classification_2}. We also evaluated adapted approaches like ML-$k$NN \cite{MLkNN_ALazyLearningApproach}, and deep learning models like Bi-LSTM \cite{bi_lstm_BidirectionalRecurrentNeuralNetworks}, and BERT \cite{bert_base_BertPretrainingOfDeepBidirectionalTransformers}. 

%\subsubsection{OVR-SVM}
%\label{subsubsec:ovr_svm}
\begin{inparaenum}[(a)]
\item\bf{One-Vs-Rest} is a heuristic method that works by decomposing the multi-label classification problem into multiple independent binary classification problems (one per class) \cite{multilabel_decomp_1_MultilabelClassificationAnOverview, multilabel_decomp_3_ATutorialOnMultilabelClassification}. It trains a single classifier per class, with the samples of that class as positive samples and all other samples as negatives. All the independent classifiers then separately give individual class predictions for unseen data. We evaluated One-Vs-Rest (OVR) approach with SVM (as the base estimator) for detecting documentation smells. One-Vs-Rest support vector machine (OVR-SVM) has been successfully applied in several problems \cite{SVM_multi_1_AKernelMethodForMultilabelled, SVM_multi_2_TextCategorizationWithSVM, multilabel_decomp_1_MultilabelClassificationAnOverview}. We used RBF kernel for the SVM classifiers as recommended by earlier works \cite{svm_rbf_1_AComparisonStudyOfDifferentKernelFunctions, svm_rbf_2_APracticalGuideToSVM}.

%\subsubsection{LPS-SVM}
%\label{subsubsec:lps_svm}
\item\bf{Label Power Set (LPS)} treats every combination of labels as a new class and approaches in a multiclass classification manner \cite{LearningMultiLabelSceneClassification}. As a result, this method has high computational complexity. However, it is capable of taking label correlation into account. We used SVM (with RBF kernel) as the base estimator of the Label Power Set method \cite{SVM_multi_1_AKernelMethodForMultilabelled, SVM_multi_2_TextCategorizationWithSVM}.


%\subsubsection{CC-SVM}
%\label{subsubsec:cc_svm}
\item\bf{Classifier Chains (CC)} constructs a chain of binary classifiers, where every classifier uses the predictions of all the previous classifiers of the chain \cite{CC_1_ClassifierChainsForMultilabel, CC_2_ClassifierChainsForMultilabel}. This way the method can take label correlations into account. We constructed a Classifier Chain (CC) of SVMs and evaluated its’ performance for documentation smell detection.



%\subsubsection{ML-$k$NN}
%\label{subsubsec:ml_knn}
\item\bf{Multi-label $k$ Nearest Neighbors (ML-$k$NN)} is derived from the traditional $k$-nearest neighbor ($k$NN) algorithm \cite{MLkNN_ALazyLearningApproach}. It finds the $k$ nearest neighborhood of an input instance using $k$NN, then uses Bayesian inference to determine the label set of the instance. We studied this method because it has been reported to achieve considerable performance for different multi-label classification tasks in previous studies \cite{MLkNN_ALazyLearningApproach, mlknn_MultilabelTextClassificationUsingSemanticFeatures}. We used ML-$k$NN with the number of nearest neighbors, $K$ = 10 during our experiment as recommended by \cite{mlknn_MultilabelTextClassificationUsingSemanticFeatures}.

\end{inparaenum}

\subsubsection{Studied Features} In this subsection, we describe the features that we used to train our SVM and \it{k}NN-based models (see section \ref{subsubsec:ovr_svm} to \ref{subsubsec:ml_knn}) for documentation smell detection.

use two types of features: the rule-based metrics, bag-of-words (as a proxy of word embeddings which will be used in BERT/LSTM - you need to 
ensure that reviewers are convinced that you have looked at each option before claiming BERT is a the best classifier)

%%%% Table %%%%%%%%%
%%%%%%%%%%%%%%%%%%%
%%%% Table %%%%%%%%%
%%%%%%%%%%%%%%%%%%%
\subsubsection{Results}

Table \ref{table_overall_performance} represents the performance of the ML models for detecting documentation smell as a multi-label classification problem. We observe that OneVsRest (OVR) and Classifier Chain (CC) achieved equal results. CC-based models are generally superior to OVR-based models because of the capability of capturing label correlation. Since the labels (types) of the documentation smells are not correlated, the CC-based SVM could not exhibit higher performance than the OVR-based SVM. However, Label Powerset (LPS) achieved lower performance than the OVR and CC-based models. To show better results, LPS-based SVM would require sufficient instances for all 32 classes of 5 smell types. Deep learning-based models like Bi-LSTM and BERT, on the other hand, outperformed the SVM and $k$NN-based models by achieving higher exact match ratios. Although Bi-LSTM showed higher Hamming loss, BERT achieved similar to the SVM and $k$NN-based models. Therefore, in terms of Hamming loss, deep learning-based models did not show any improvement. However, considering both exact match ratio and Hamming loss as the performance metrics, we can deduce that BERT is the most suitable of all the models experimented in detecting the documentation documentation smell.
\begin{table}[t]
\caption{Shallow models on the overall smell types detection}
\centering
%\begin{center}
%\scalebox{1.0}
%\resizebox{\columnwidth}{!} %new add
%{
%\renewcommand*{\arraystretch}{2}
\begin{tabular}{lrr}
\toprule
\textbf{Model}   & \textbf{Exact Match Ratio} & \textbf{Hamming Loss} \\ \midrule
\textbf{Rule-based} & .17                        & .35       \\ %\hline
\textbf{OVR-SVM} & .50                        & \textbf{.14}          \\ %\hline
\textbf{LPS-SVM} & .48                        & .15                   \\ %\hline
\textbf{CC-SVM}  & .50                        & \textbf{.14}          \\ %\hline
\textbf{ML-$k$NN}  & .47                        & .15                   \\ %\hline
%\textbf{Bi-LSTM} & .80                        & .20                   \\ %\hline
%\textbf{BERT}    & \textbf{.84}               & .15                   \\ 
\bottomrule
\end{tabular}
%}
\label{table_overall_performance}
%\end{center}
\end{table}
\begin{table*}[t]
\caption{Performance on different type of documentation smells}
%\begin{center}
%\scalebox{1.0}
%{
%\renewcommand*{\arraystretch}{3}
\begin{tabular}{lrrrr|rrrr|rrrr|rrrr|rrrr}
%                                       & \multicolumn{20}{c}{}                                         \\ \cmidrule{2-21} 
\multicolumn{1}{l}{}                  & \multicolumn{4}{c}{\textbf{Bloated}}                                                                     & \multicolumn{4}{c}{\textbf{Lazy}}                                                                        & \multicolumn{4}{c}{\textbf{Excess   Struct}}                                                             & \multicolumn{4}{c}{\textbf{Tangled}}                                                                     & \multicolumn{4}{c}{\textbf{Fragmented}}                                                                  \\ 
\midrule
{\textbf{Model}}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}  \\ 
\midrule
{\textbf{Rule-based}} & {.76} & {.67} & {.86} &{.75} & {.57} & {.69} & {.70} &{.69} & {.74} & {.68} & {.74} &{.71} & {.51} & {.40} & {.38} &{.39} & {.61} & {.57} & {.58} &{.58} \\ %\hline
{\textbf{OVR-SVM}} & {\textbf{.97}} & {.88} & {.89} &{.89} & {.93} & {.85} & {.92} &{.88} & {\textbf{.77}} & {.48} & {.23} &{.31} & {\textbf{.85}} & {.72} & {.54} &{.62} & {\textbf{.76}} & {\textbf{.77}} & {.44} &{.56} \\ %\hline
{\textbf{LPS-SVM}} & {.96} & {.90} & {.77} &{.83} & {.94} & {.84} & {.96} &{.89} & {\textbf{.77}} & {.50} & {.24} &{.33} & {.83} & {.71} & {.42} &{.54} & {.73} & {.64} & {.49} &{.56} \\ %\hline
{\textbf{CC-SVM}}  & {\textbf{.97}} & {.88} & {.90} &{.89} & {.93} & {.83} & {.93} &{.87} & {\textbf{.77}} & {.49} & {.21} &{.29} & {\textbf{.85}} & {.72} & {.54} &{.62} & {\textbf{.76}} & {.75} & {.45} &{.56} \\ %\hline
{\textbf{ML-$k$NN}}  & {.95} & {.77} & {.82} &{.80} & {.91} & {.83} & {.84} &{.84} & {.76} & {.46} & {.39} &{.42} & {.82} & {.65} & {.55} &{.60} & {\textbf{.76}} & {.65} & {.64} &{.65} \\ %\hline
\bottomrule
%{\textbf{Bi-LSTM}} & {.92} & {.92} & {.92} &{.91} & {.89} & {.90} & {.89} &{.90} & {.76} & {.72} & {\textbf{.76}} &{.73} & {.78} & {.74} & {.78} &{.74} & {.67} & {.64} & {.67} &{.63} \\ %\hline
%{\textbf{BERT}}    & {.93} & {\textbf{.93}} & {\textbf{.93}} &{\textbf{.93}} & {\textbf{.97}} & {\textbf{.97}} & {\textbf{.97}} &{\textbf{.97}} & {.76} & {\textbf{.75}} & {\textbf{.76}} &{\textbf{.76}} & {.83} & {\textbf{.83}} & {\textbf{.83}} &{\textbf{.83}} & {.75} & {.75} & {\textbf{.75}} &{\textbf{.75}} \\ 
%\hline
\end{tabular}
%}
\label{table_individual_performance}
%\end{center}
\end{table*}
%%%% Table %%%%%%%%%
%%%%%%%%%%%%%%%%%%%
\subsubsection{Results}
Table \ref{table_individual_performance} shows the performance of the ML models
on each type of documentation smells. Although SVM and $k$NN-based models
achieved slightly better accuracy than Bi-LSTM and BERT, the later models
outperformed SVM and $k$NN-based models in F1-score. This behavior is due to the
unequal distribution of the smell types over the dataset. SVM and $k$NN-based
models produced more false-negative results because the number of positive
instances for an individual smell type is significantly lower than the number of
negative instances for that type. As a result, SVM and $k$NN-based models showed
quite low recalls for some types (Excess Struct, Tangled, and Fragmented) and
consequently resulted in low F1-scores. 
%\subsubsection{Feautre Importance Analysis}
\gias{TODO: do the feature-based analysis here, i.e., ablation study on the shallow learning models as discussed}

\subsection{Can the deep machine learning models outperform the shallow learning models? (RQ3)}
\subsubsection{Deep Learning Models}
%\subsubsection{Bi-LSTM}
Bidirectional LSTM is more capable of exploiting contextual information than the unidirectional LSTM \cite{bilstm_FramewisePhonemeClassificationWithBiLSTM}. Hence, the Bi-LSTM network can detect the documentation smell by capturing the information of the API documentations from both directions. We constructed a Bi-LSTM model with 300 hidden states and initialized it using the pre-trained GloVe embedding \cite{Glove_GlobalVectorsForWordRepresentation} of 100 dimensions. We used ADAM optimizer \cite{adam_optimizer} with an initial learning rate of 0.001. We trained the model with batch size 256 over 10 epochs.


%\subsubsection{BERT}
Considering the great success of BERT (Bidirectional Encoder Representations from Transformers) in various natural language processing and text classification tasks \cite{bert_success_1,bert_success_2,bert_success_3,bert_success_4,bert_success_5,bert_success_6,bert_success_7}, we feel motivated to evaluate its’ performance in documentation smell detection. BERT is a  pre-trained model which was designed to learn contextual word representations of unlabeled texts \cite{bert_base_BertPretrainingOfDeepBidirectionalTransformers}. We used BERT-Base for this study which has 12 layers with 12 attention heads and 110 million parameters. We trained it on our labeled dataset for 10 epochs with a mini-batch size of 32. We used early-stop to avoid overfitting \cite{early_stop_bert_1} and considered validation loss as the metric of the early-stopping \cite{early_stop_bert_2}. The maximum length of the input sequence was set to 256. We used AdamW optimizer \cite{adam_w} with the learning rate set to 4e\textsuperscript{-5}, ß1 to 0.9, ß2 to 0.999, and epsilon to 1e\textsuperscript{-8} \cite{bert_base_BertPretrainingOfDeepBidirectionalTransformers, bert_fine_tuning}. We used binary cross-entropy to calculate the loss \cite{binary_cross_AreLossFunctionSame}. 


\subsubsection{Studied Features} talk about word-embeddings

\subsubsection{Results}
On the other hand, Bi-LSTM and BERT
focused on capturing generalized attributes for each smell type and as a result,
achieved impressive performance in all the performance metrics. Overall, BERT
showed promising results among all the models in accurately detecting each of
the individual documentation smells.
\begin{table}
\begin{tabular}{lrr}
\toprule
\textbf{Model}   & \textbf{Exact Match Ratio} & \textbf{Hamming Loss} \\ \midrule

%\textbf{Rule-based} & .17                        & .35       \\ %\hline
%\textbf{OVR-SVM} & .50                        & \textbf{.14}          \\ %\hline
%\textbf{LPS-SVM} & .48                        & .15                   \\ %\hline
%\textbf{CC-SVM}  & .50                        & \textbf{.14}          \\ %\hline
%\textbf{ML-$k$NN}  & .47                        & .15                   \\ %\hline
\textbf{Bi-LSTM} & .80                        & .20                   \\ %\hline
\textbf{BERT}    & \textbf{.84}               & .15                   \\ %\hline
\bottomrule
\end{tabular}
%}
\label{table_overall_performance}
%\end{center}
\end{table}

% \begin{table*}[!ht]
% \caption{Performance on different type of documentation smells}
% \begin{center}
% \scalebox{1.0}
% {
% %\renewcommand*{\arraystretch}{3}
% \begin{tabular}{ccccccccccccccccccccc}
%                                        & \multicolumn{20}{c}{}                                         \\ \cline{2-21} 
%{}                  & \multicolumn{4}{c|}{\textbf{Bloated}}                                                                     & \multicolumn{4}{c|}{\textbf{Lazy}}                                                                        & \multicolumn{4}{c|}{\textbf{Excess   Struct}}                                                             & \multicolumn{4}{c|}{\textbf{Tangled}}                                                                     & \multicolumn{4}{c|}{\textbf{Fragmented}}                                                                  \\ \hline
% {\textbf{Model}}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}  \\ \hline
% %{\textbf{Rule-based}} & {.76} & {.67} & {.86} &{.75} & {.57} & {.69} & {.70} &{.69} & {.74} & {.68} & {.74} &{.71} & {.51} & {.40} & {.38} &{.39} & {.61} & {.57} & {.58} &{.58} \\ %\hline
% %{\textbf{OVR-SVM}} & {\textbf{.97}} & {.88} & {.89} &{.89} & {.93} & {.85} & {.92} &{.88} & {\textbf{.77}} & {.48} & {.23} &{.31} & {\textbf{.85}} & {.72} & {.54} &{.62} & {\textbf{.76}} & {\textbf{.77}} & {.44} &{.56} \\ %\hline
% %{\textbf{LPS-SVM}} & {.96} & {.90} & {.77} &{.83} & {.94} & {.84} & {.96} &{.89} & {\textbf{.77}} & {.50} & {.24} &{.33} & {.83} & {.71} & {.42} &{.54} & {.73} & {.64} & {.49} &{.56} \\ %\hline
% %{\textbf{CC-SVM}}  & {\textbf{.97}} & {.88} & {.90} &{.89} & {.93} & {.83} & {.93} &{.87} & {\textbf{.77}} & {.49} & {.21} &{.29} & {\textbf{.85}} & {.72} & {.54} &{.62} & {\textbf{.76}} & {.75} & {.45} &{.56} \\ %\hline
% %{\textbf{ML-$k$NN}}  & {.95} & {.77} & {.82} &{.80} & {.91} & {.83} & {.84} &{.84} & {.76} & {.46} & {.39} &{.42} & {.82} & {.65} & {.55} &{.60} & {\textbf{.76}} & {.65} & {.64} &{.65} \\ %\hline
% {\textbf{Bi-LSTM}} & {.92} & {.92} & {.92} &{.91} & {.89} & {.90} & {.89} &{.90} & {.76} & {.72} & {\textbf{.76}} &{.73} & {.78} & {.74} & {.78} &{.74} & {.67} & {.64} & {.67} &{.63} \\ %\hline
% {\textbf{BERT}}    & {.93} & {\textbf{.93}} & {\textbf{.93}} &{\textbf{.93}} & {\textbf{.97}} & {\textbf{.97}} & {\textbf{.97}} &{\textbf{.97}} & {.76} & {\textbf{.75}} & {\textbf{.76}} &{\textbf{.76}} & {.83} & {\textbf{.83}} & {\textbf{.83}} &{\textbf{.83}} & {.75} & {.75} & {\textbf{.75}} &{\textbf{.75}} \\ \hline
% \end{tabular}
% }
% \label{table_individual_performance}
% \end{center}
% \end{table*}
\begin{table*}[t]
\caption{Performance on different type of documentation smells}
%\begin{center}
%\scalebox{1.0}
%{
%\renewcommand*{\arraystretch}{3}
\begin{tabular}{lrrrr|rrrr|rrrr|rrrr|rrrr}
%                                       & \multicolumn{20}{c}{}                                         \\ \cmidrule{2-21} 
\multicolumn{1}{l}{}                  & \multicolumn{4}{c}{\textbf{Bloated}}                                                                     & \multicolumn{4}{c}{\textbf{Lazy}}                                                                        & \multicolumn{4}{c}{\textbf{Excess   Struct}}                                                             & \multicolumn{4}{c}{\textbf{Tangled}}                                                                     & \multicolumn{4}{c}{\textbf{Fragmented}}                                                                  \\ 
\midrule
{\textbf{Model}}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}   & {A}   & {P}   & {R}   &{F1}  \\ 
\midrule
{\textbf{Bi-LSTM}} & {.92} & {.92} & {.92} &{.91} & {.89} & {.90} & {.89} &{.90} & {.76} & {.72} & {\textbf{.76}} &{.73} & {.78} & {.74} & {.78} &{.74} & {.67} & {.64} & {.67} &{.63} \\ %\hline
{\textbf{BERT}}    & {.93} & {\textbf{.93}} & {\textbf{.93}} &{\textbf{.93}} & {\textbf{.97}} & {\textbf{.97}} & {\textbf{.97}} &{\textbf{.97}} & {.76} & {\textbf{.75}} & {\textbf{.76}} &{\textbf{.76}} & {.83} & {\textbf{.83}} & {\textbf{.83}} &{\textbf{.83}} & {.75} & {.75} & {\textbf{.75}} &{\textbf{.75}} \\ 
\bottomrule
\end{tabular}
%}
\label{table_individual_performance}
%\end{center}
\end{table*}
\gias{TODO. Now report some misclassified cases of BERT per documentation smell and explain why the misclassification occurred.}

\subsection{Can the detection of one documentation smell support the detection another smell? (RQ4)}
In multi-label learning, the labels might be interdependent and correlated \cite{label_correlation_paper_1}. We used Phi Coefficients to determine such interdependencies and correlations between different documentation smells. The Phi Coefficient is a measure of association between two binary variables \cite{phi_coefficient_paper}. It ranges from -1 to +1, where ±1 indicates a perfect positive or negative correlation, and 0 indicates no relationship. We report the Phi Coefficients between each pair of labels in Figure \ref{fig:label_correlation}. We find that there is almost no correlation between `Fragmented’ and any other smell (except `Lazy’). By definition, the information of fragmented documentation is scattered in many sections or pages. Hence, it has little to do with smells like `Bloated’, `Excess Structural Information’, `Tangled’. We also observe that there is a weak positive correlation (+0.2 to +0.4) among the `Bloated’, `Excess Structural Information’, and `Tangled’ smells. One possible reason might be that if a documentation is filled with complex and unorganized information (Tangled), and unnecessary structural information (Excess Structural Information), it might be prone to become bloated as well. On the other hand, `Lazy’ smell has a weak negative correlation (-0.2 to -0.3) with all other groups since these kinds of documentation are often too small to contain other smells. However, none of these coefficients is high enough to imply a strong or moderate correlation between any pair of labels. Hence, it justifies our catalog by indicating that all the smells that we proposed are sufficiently unique in nature.

\begin{figure}[t]%[!htb]
  \centering
  %\vspace{-6mm}
   \hspace*{-.7cm}%
  \includegraphics[scale=.5]{new_images/label_correlation.png}
 % \vspace{-4mm}
  \caption{Correlation of different documentation smells. Red, Blue, and Gray mean positive, negative, and no correlation respectively. Intensity of color indicates the level of correlation.}

  \label{fig:label_correlation}
%\vspace{-4mm}
\end{figure}


% 
% \subsection{Ablation Study (RQ4)}
% BERT - epoch change
% SVM - feature change.



%\subsection{How accurate is each feature dimension?}
%answer RQ

%\subsection{How well does hypertuning work in the ML models?}
%answer RQ.


==> study-results.tex <==
\section{Study Results}
In this section, we present the results organized by the research questions. 
\subsection{How accurately can we detect TDs in R packages? (RQ1)}
\label{subsec:rq1}
\subsubsection{Motivation}
motivation of rq1
\subsubsection{Approach}
We developed a two-stage framework to detect TD instances of a package from corresponding GitHub issue comments as depicted in Figure \ref{fig:td_type_detection_workflow}. For a given issue comment, we split it into sentences and every sentence is labeled as TD significant or insignificant in stage-1. TD insignificant sentences are discarded and the TD significant sentences are passed to stage-2 for TD-type detection. The detailed workflow of the two stages are mentioned below.

\begin{figure*}[t]
  \centering
  %\vspace{-6mm}
   %\hspace*{-.7cm}%
  %\includegraphics[scale=0.7]{new_images/td_type_detection.png}
  \includegraphics[height=3.5cm, width=16cm]{new_images/td_type_detection.png}
 % \vspace{-4mm}
  \caption{Correlation between different types of TD in R packages. Intensity of (red) color indicates the level of correlation.}

  \label{fig:td_type_detection_workflow}
\vspace{-1mm}
\end{figure*}

\textbf{Discarding Insignificant Sentences.}
In the first stage, we developed a BERT-based model that would detect TD-significant vs TD-insignificant instances in a binary classification fashion. BERT is a pre-trained model which was designed to learn contextual word representations of unlabeled texts \cite{Delvin-BERTArch-Arxiv2018}. We chose BERT because it is found to significantly outperform other models in various natural language processing and text classification tasks \cite{bert_success_1,bert_success_2,bert_success_3,bert_success_4,bert_success_5,bert_success_6,bert_success_7}. We used BERT-Base containing 12 layers with 12 attention heads and 110 M parameters. We appended a classification head composed of a single linear layer on top of it. For this stage, we used our binary fashioned dataset (i.e. consisting two labels: TD and non-TD). We first split the dataset in 80:20 ratio to create train and test sets, Then we trained the model with the train set for 10 epochs with
a mini-batch size of 32 and maximum input length of 300. We used early-stop to avoid overfitting
\cite{early_stop_bert_1} considering validation loss as the metric of the
early-stopping \cite{early_stop_bert_2}. We used AdamW optimizer \cite{adam_w} setting the learning
rate to 4e\textsuperscript{-5}, $\beta1$ to 0.9, $\beta2$ to 0.999, and $\epsilon$ to
1e\textsuperscript{-8}
\cite{Delvin-BERTArch-Arxiv2018, bert_fine_tuning}. We used binary cross-entropy to calculate the loss \cite{binary_cross_AreLossFunctionSame}. We refer to this model as \textbf{S1M (Stage-1 Model)} for the rest of this paper.

\textbf{Detection of TD-type.}
In this stage, we want to detect the type of TD from a given instance (i.e. sentence). We consider ten types of TD discussed in \cite{codabux2021technical}. Hence, it is a 10-class classification problem. We first evaluated the effectiveness of a single classifier to decide among all the 10 possible classes. However, the single classifier performed very poorly on the classification task with an accuracy of $\sim$12\% which is nearly random for a 10-class problem. In the multi-class scenario, the classification task becomes very difficult since the classifier has to distinguish between a large number of classes in order to make predictions. To deal with this issue, we leveraged the concept of hierarchical classification \cite{arabie1996hierarchical,silla2011survey}. Hierarchical classification approaches the multi-class problem by splitting the output space like a tree where each (parent) node is divided into a number of child nodes, and the procedure is repeated until each child node represents a single class \cite{chaitra2018review}. Hence, it needs a predefined data taxonomy according to which it hierarchically distributes all the classes in a collection of multi-class sub-problems and thus the number of classes involved in each local sub-problem gets reduced. To induce the class hierarchy (i.e. taxonomy), we followed the procedure proposed by Daniel et al. \cite{confusionMatrix_for_hierarchy}. We used the $10\times10$ confusion matrix produced while using a single classifier to predict among all 10 classes together. First, we generated a distance matrix $(D)$ from the confusion matrix $(M)$ using the steps showed in Figure \ref{fig:generating_distance_matrix}. Any element of the distance matrix, $D(i,j)$ indicates the level of similarity between the class $i$ and $j$ ranging from 0 to 1 where 0 (and 1) means completely indistinguishable (and distinguishable). Then we divided all 10 types of TD in 3 clusters using spectral clustering algorithm \cite{spectralCluster1, spectralCluster2}. The optimal number of cluster, K (=3) was determined using eigengap heuristic \cite{spectralCluster2}. Thus, we induced a hierarchy of TD types as showed in Figure \ref{TD_Hierarchy_fig}. Then we used a total of 4 BERT-based classifiers (each for every parent node) where the first classifier (of the root node) was trained to distinguish among the three clusters only. To achieve this goal, we relabeled all the data of our dataset into three classes according to the hierarchy of Figure \ref{TD_Hierarchy_fig} and trained the first classifier on it. We call it \textbf{S2M0 (Stage-2 Model-0)}. Similarly, the next three classifiers (addressed later as \textbf{S2M1, S2M2, S2M3}) were trained to detect debts of Cluster-1, Cluster-2, and Cluster-3 respectively. Hence, \textbf{S2M1} detects among documentation, code, defect, test, and design debts; \textbf{S2M2} detects among build, architecture, and versioning debts; \textbf{S2M3} detects among usability and requirement debts.


\begin{figure}[t]%[!htb]
  \centering
  %\vspace{-6mm}
  %\hspace*{-.7cm}%
   \includegraphics[scale=.5]{new_images/distance_matrix.png}
 % \vspace{-4mm}
  \caption{Generating distance matrix (D) from confusion matrix (M) following \cite{confusionMatrix_for_hierarchy}}

  \label{fig:generating_distance_matrix}
\vspace{-4mm}
\end{figure}


\begin{figure*}
\centering
\begin{forest}
for tree={%
    edge path={\noexpand\path[\forestoption{edge}] (\forestOve{\forestove{@parent}}{name}.parent anchor) -- +(0,-12pt)-| (\forestove{name}.child anchor)\forestoption{edge label};}
}
[
{TD Type}
[
Cluster-1
[Documentation]
[Code]
[Defect]
[Test]
[Design]
]
[
Cluster-2
[Build]
[Architecture]
[Versioning]
]
[
Cluster-3
[Usability]
[Requirement]
]
]
\end{forest}

\caption{Hierarchy of different types of TD}
\label{TD_Hierarchy_fig}
\end{figure*}

% \textbf{Example.} To predict the TD presence and type in a given issue comment, we first split the comment into sentences. In the first stage of our framework, we predict the presence of TD in each sentence (i.e. whether the sentence is TD significant or not). Only the TD significant sentences will enter the second stage for type detection. For example, if all the sentences 

\textbf{Evaluation Metrics.}
We report the performances of our classifiers using four standard metrics: Accuracy, Precision, Recall, F1-score \cite{Manning-IRIntroBook-Cambridge2009}. Accuracy ($A$) is the ratio of the number of 
correctly predicted examples out of all data. Precision ($P$) is the ratio of the number of correctly predicted examples and all the predicted examples for a given class.
Recall ($R$) is  the ratio of the number of correctly predicted examples and  all  examples of a given class. F1-score ($F1$) is the harmonic mean of
precision and recall.

{\scriptsize
\begin{eqnarray*}
P  = \frac{TP}{TP+FP},~
R = \frac{TP}{TP+FN},~
F1 = 2*\frac{P*R}{P+R},~
A = \frac{TP+TN}{TP+FP+TN+FN}
\end{eqnarray*}}
TP = Correctly classified as a TD, 
FP = Incorrectly classified as a TD, TN = Correctly classified as not a TD, 
FN = Incorrectly classified as not a TD. 

\subsubsection{Results}
In stage-1, we developed a binary classification model (S1M) for discarding TD insignificant sentences from an issue comment. It detects the presence of TD with 94\% accuracy and 92\% F1-score. Since the task of stage-1 (i.e. binary classification) is relatively simple and straight-forward, state-of-the-art pre-trained language model like BERT shows high performance here \cite{bert_success_1, bert_success_2,bert_success_6,bert_success_7}. On the other hand, almost all of the tasks of stage-2 are multi-class problems (except S2M3). Hence, we see a downgrade of performance in this stage, specially S2M1 which has to distinguish among 5 classes of cluster-1 (i.e.documentation, code, defect, test, design debts). It achieves 72\% accuracy with 71\% F1-score. Other models of stage-2 i.e. S2M0, S2M2, S2M3 show better performance with F1-scores of 81\%, 77\%, and 90\% respectively. Since cluster-3 contains only 2 classes (i.e. usability, requirement debts), the classification becomes binary problem and S2M3 achieves better performance than other models.        

\begin{table}
\centering
\caption{Performance of automatic TD detection.}
\scalebox{1}
{
\begin{tabular}{@{}lcccccc@{}}
\toprule
\textbf{\begin{tabular}[c]{@{}l@{}}Model\\ Type\end{tabular}} & \textbf{Stage}                                & \textbf{\begin{tabular}[c]{@{}c@{}}Model \\ Name\end{tabular}} & \textbf{A} & \textbf{P} & \textbf{R} & \textbf{F} \\ \midrule
\multicolumn{1}{l|}{\multirow{5}{*}{BERT}}                    & \multicolumn{1}{c|}{Stage-1}                  & \multicolumn{1}{c|}{S1M}                                       & 0.94       & 0.92       & 0.91       & 0.92       \\ \cmidrule(l){2-7} 
\multicolumn{1}{l|}{}                                         & \multicolumn{1}{c|}{\multirow{4}{*}{Stage-2}} & \multicolumn{1}{c|}{S2M0}                                      & 0.86       & 0.82       & 0.80       & 0.81       \\
\multicolumn{1}{l|}{}                                         & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{S2M1}                                      & 0.72       & 0.73       & 0.70       & 0.71       \\
\multicolumn{1}{l|}{}                                         & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{S2M2}                                      & 0.77       & 0.77       & 0.76       & 0.77       \\
\multicolumn{1}{l|}{}                                         & \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{S2M3}                                      & 0.91       & 0.93       & 0.88       & 0.90       \\ \bottomrule
\end{tabular}
}
\label{table_model_performance}
\end{table}



\subsection{How prevalent are TDs in R packages? (RQ2)}
\subsubsection{Motivation}
TD are different in types, characteristics, and distribution. They have different causes and consequences. Hence, one TD can occur more (or less) frequently than the others. Moreover, the level of concern of developers as well as the reviewers might vary from one type to another. To comprehend such differences in the prevelance of TD, we want to determine the distribution of different types.
\subsubsection{Approach}
We used the data collected in section \ref{sec:data_collection} for our empirical study. We determined the TD types indicated in all the issue comments collected from rOpenSci and BioConductor packages using our automatic framework developed in RQ1. One issue comment can indicate one or more types of TD at different sentences or phrases. Since we are using sentence level detection, our framework is able to catch all of the types expressed in each issue comment. We counted all the TD instances of different types both for rOpenSci and BioConductor packages, then showed their distribution using bar chart.  

\subsubsection{Results}
Figure \ref{fig:TD_distribution_rOpenSci} and Figure \ref{fig:TD_distribution_BioConductor} depict the distribution of different types of TD in rOpenSci and BioConductor respectively. We find a total of 3938 TD instances in $\sim$4.5K issue comments of rOpenSci and 10159 TD instances in $\sim$9K issue comments of BioConductor. However, not all types of TDs are equally prevalent in R packages. Among all the types, documentation debt is the most frequent one with 938 occurrences ($\sim$23.8\%) in rOpenSci and 2740 occurrences ($\sim$27\%) in BioConductor. On the other side, versioning debt is the least prominent one with only 22 occurrences in rOpenSci and 71 occurrences in BioConductor. Apart from documentation debt, some other TD such as design debt, defect debt, and code debt occur frequently. Moreover, we see almost similar distribution of different TDs for both rOpenSci and BioConductor packages which suggests that different types of TDs occur in similar distribution in R packages regardless of the platform, scope, and field.   


\begin{figure}[t]%[!htb]
  \centering
  %\vspace{-6mm}
  %\hspace*{-.7cm}%
   \includegraphics[scale=.19]{new_images/TD_distribution_rOpenSci.png}
 % \vspace{-4mm}
  \caption{Distribution of different TDs in rOpenSci.}

  \label{fig:TD_distribution_rOpenSci}
\vspace{-4mm}
\end{figure}


\begin{figure}[t]%[!htb]
  \centering
  %\vspace{-6mm}
  %\hspace*{-.7cm}%
   \includegraphics[scale=.19]{new_images/TD_distribution_BioConductor.png}
 % \vspace{-4mm}
  \caption{Distribution of different TDs in BioConductor.}

  \label{fig:TD_distribution_BioConductor}
\vspace{-4mm}
\end{figure}



\subsection{How do the TDs evolve in R packages? (RQ3)}
\subsubsection{Motivation}
Trend analysis allows us to see how things got to where they are now and predict how they might change in the future. It's natural that different TD grow at different rates and trends. For example, any specific type could increase (or decrease) quicker (or slower) than the others. To capture such notions, we examined how different TD evolve over time which will assist the developers, users, and reviewers to understand how and why things are changing as well as what to expect next.
\subsubsection{Approach}
\label{subsub:RQ3_Approach}
To investigate how different types of TD evolve over time, we conducted a year-wise trend analysis. For each type, we divided the total number of TD instances detected in a year by the total number of packages in that year. Thus we determined the average number of TD (per package) over years and plotted them in the graph. Depending on the availability of data, we considered the packages from April 2015 to April 2020 for the trend analysis of rOpenSci and from April 2016 to April 2021 for BioConductor. To get an overall idea about the growth of different types of TD, we also calculated the overall change in the occurrence and the compound annual growth rate (CAGR) for each TD type combining the data of both rOpenSci and BioConductor over years 2016--2020.

\subsubsection{Results}
Figure \ref{fig:trend_rOpenSci} and \ref{fig:trend_BioConductor} show the trend analysis of rOpenSci and BioConductor packages respectively. For rOpenSci, we see an overall upward trend for most types of TD (except the architecture debt). Among them, documentation debt has the most overall per package increment of $\sim$2.5 unit over five years starting at $\sim$4.5 debts in 2015 and reaching $\sim$7 in 2020 with a steep slope at the tail (Figure \ref{fig:trend_rOpenSci}). It indicates the constantly growing concern of the reviewers and users regarding documentation quality. Defect and test debts are two other types with significant increment of 1.6 and 1.4 unit per package throughout this time. On the other hand, we see a decreasing trend in architecture debt with less than 1 unit (per package) in 2020. Literature suggests that unlike other TD (such as code-level technical debt), architecture debt is very difficult to detect as they do not show any clear symptom \cite{verdecchia2020architectural, verdecchia2021building}. So it might happen that with growing diversity and complexity of packages, it is gradually becoming more challenging to identify architecture debts. For BioConductor, we see an overall downward trend for all types of TD. Even for the most prevalent type (i.e. documentation debt), the per package number has dropped below 2 in 2021 while in 2016 it was close to 3 (Figure \ref{fig:trend_BioConductor}). Since BioConductor is a domain-specific platform, the packages might have fewer sources of debts compared to rOpenSci.        


\begin{figure}[t]%[!htb]
  \centering
  %\vspace{-6mm}
  %\hspace*{-.7cm}%
   \includegraphics[scale=.19]{new_images/Trend_rOpenSci.png}
 % \vspace{-4mm}
  \caption{Trend analysis of different TD in rOpenSci packages.}

  \label{fig:trend_rOpenSci}
\vspace{-4mm}
\end{figure}


\begin{figure}[t]%[!htb]
  \centering
  %\vspace{-6mm}
  %\hspace*{-.7cm}%
   \includegraphics[scale=.19]{new_images/Trend_BioConductor.png}
 % \vspace{-4mm}
  \caption{Trend analysis of different TD in BioConductor packages.}

  \label{fig:trend_BioConductor}
\vspace{-4mm}
\end{figure}


\begin{table}
\centering
\caption{Growth-rate of different types of TD.}
\scalebox{1}
{
\begin{tabular}{@{}lcr@{}}
\toprule
\textbf{TD Type} &  $\Delta$\textbf{Occurrence} & \textbf{Growth Rate (\%)} \\ \midrule
Documentation    & 2.14                & 5.41                      \\
Build            & 0.45                & 3.78                      \\
Requirement      & 0.61                & 3.42                      \\
Architecture     & -0.75               & -7.15                     \\
Design           & 0.17                & 0.52                      \\
Usability        & 0.05                & 1.77                      \\
Code             & 0.74                & 3.82                      \\
Versioning       & -0.03               & -5.58                     \\
Test             & 1.28                & 15.05                     \\
Defect           & 1.24                & 5.84                      \\ \bottomrule
\end{tabular}
}
\label{table:td_growth_rate}
\end{table}



% \subsection{How do developers find information about TDs useful? (RQ4)}
% \subsubsection{Motivation} motivate
% \subsubsection{Approach} approach
% \subsubsection{Results} results


==> study-setup.tex <==
\section{Study Setup}
%\subsection{Goal and Research Questions}
\subsection{Schematic Overview}
overview of methodology

\begin{figure*}[t]
  \centering
  %\vspace{-6mm}
   %\hspace*{-.7cm}%
  %\includegraphics[scale=0.7]{new_images/td_type_detection.png}
  \includegraphics[scale=.7]{new_images/Schematic Overview6}
 % \vspace{-4mm}
  \caption{Schematic diagram of our study.}

  \label{fig:schematic_digram}
\vspace{-1mm}
\end{figure*}

\subsection{Dataset Preparation}

\subsubsection{Data Collection} \label{sec:data_collection}
We collected over 13.5K review comments with $\sim$4.5K issue comments coming from 173 approved rOpenSci packages\footref{ropensci_footnote} and $\sim$9K from 1124 approved BioConductor packages\footnote{\url{https://www.bioconductor.org/}} to conduct our empirical study. We extracted these issue comments from respective GitHub repositories of each platforms\footnote{\url{https://github.com/ropensci}}\footnote{\url{ https://github.com/Bioconductor}} using web crawling and text parsing techniques. We chose only the approved packages to ensure the completeness of the review process and the standard of the packages so that we can get a legitimate view of the TD from our study.  

%\gias{justify why you only collected the approved comments}



%\gias{there is a missing link between the data collection above and the this dataset. I understand that this Zadia et al. dataset is also included in the 13.5K comments above, but a reviewer might not know this. Please clarify}
\subsubsection{Labeling}
We used the dataset published by Zadia et al. \cite{codabux2021technical} which contains 600 TD instances in R peer-reviews documentation of rOpenSci manually labelled in 10 TD types. Each instance is a phrase extracted from a full issue comment through manual investigation. First, they extracted the comments of all 157 approved rOpenSci packages of that time. Note that these data are also included in the current 173 approved packages we extracted. Second, they manually investigated a randomly selected subset of the comments and identified the ones with potential TD indication. Later, 600 phrases were manually extracted from those comments and labelled in different TD types. Hence, one limitation of the dataset is that it only contains TD significant parts of the issue comments and remaining parts of the comments (i.e. insignificant/non-TD sentences) were discarded. Since issue comments are from natural human language domain, it is obvious that they contain a number of sentences that are not relevant to TD. Hence, for automatic detection, we need a number of such non-TD sentences as well for training our machine learning model so that it can distinguish them from TD sentences and discard them from a given issue comment in real world scenario. Accordingly, we built a dataset of both TD-significant and TD-insignificant sentences as follows. \begin{inparaenum}[(1)]
\item We extracted the full comments of TD instances labeled in the dataset \cite{codabux2021technical} using their comment-ids. \item We split the extracted comments into sentences. \item Among these sentences, ones that exist in the TD dataset of \cite{codabux2021technical} are considered significant for determining TD. \item The rest sentences are considered insignificant. In this process, we obtained a binary dataset of total of 1205 sentences: 805 TD significant and 400 TD insignificant (i.e. non-TD). Each of these 805 TD sentences again carries a type (i.e. TD type) as labeled in the original dataset \cite{codabux2021technical}. \end{inparaenum}


\begin{table}
\centering
\caption{Statistics of Dataset}
\begin{tabular}{llr}
\toprule
\multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}TD \\ Presence\end{tabular}}} & TD Type  & \# Sentence \\ \midrule
\multicolumn{1}{l|}{\textbf{Non-TD}}  & N/A      & 400     \\ \midrule
\multicolumn{1}{l|}{}        & Documentation       & 230     \\
\multicolumn{1}{l|}{}        & Code     & 226     \\
\multicolumn{1}{l|}{}        & Design         & 202     \\
\multicolumn{1}{l|}{}        & Defect         & 192     \\
\multicolumn{1}{l|}{\textbf{TD}}      & Requirement        & 207     \\
\multicolumn{1}{l|}{}        & Test     & 195     \\
\multicolumn{1}{l|}{}        & Architecture        & 200     \\
\multicolumn{1}{l|}{}        & Build    & 172     \\
\multicolumn{1}{l|}{}        & Usability     & 150     \\
\multicolumn{1}{l|}{}        & Versioning              & 104     \\ \midrule 
& \textbf{Total}       & 2278 \\                                                           \bottomrule            
\end{tabular}

\label{dataset_table_1}
\end{table}


% \begin{table}
% \centering
% \caption{Statistics of Dataset}
% \begin{tabular}{llrrr}
% \toprule
% \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}TD \\ Presence\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}l@{}}TD \\ Type\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Sentence \#\\ (Original)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Augmentation\\ Scale\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Sentence \#\\ (Augmented)\end{tabular}} \\ \midrule
% \multicolumn{1}{l|}{\textbf{Non-TD}}  & N/A    & 400    & 0  & 400     \\ \midrule
% \multicolumn{1}{l|}{}        & Documentation     & 230    & 0  & 230     \\
% \multicolumn{1}{l|}{}        & Code   & 113    & 1  & 226     \\
% \multicolumn{1}{l|}{}        & Design       & 101    & 1  & 202     \\
% \multicolumn{1}{l|}{}        & Defect       & 96     & 1  & 192     \\
% \multicolumn{1}{l|}{\textbf{TD}}      & Requirement       & 69     & 2  & 207     \\
% \multicolumn{1}{l|}{}        & Test   & 65     & 2  & 195     \\
% \multicolumn{1}{l|}{}        & Architecture      & 50     & 3  & 200     \\
% \multicolumn{1}{l|}{}        & Build  & 43     & 3  & 172     \\
% \multicolumn{1}{l|}{}        & Usability    & 30     & 4  & 150     \\
% \multicolumn{1}{l|}{}        & Versioning        & 8      & 12       & 104     \\ \midrule 
% & \textbf{Total}    & 1205   & N/A      & 2278 \\                                                           \bottomrule            
% \end{tabular}

% \label{dataset_table_1}
% \end{table}


\subsubsection{Data Augmentation}
One issue of the dataset is it is greatly imbalanced i.e. some types have extremely low number of instances compared to others. For example, among the 600 TD phrases of their dataset, only 5 ($\sim$0.99\%) are from versioning debts while 186 phrases ($\sim$28.5\%) are from documentation debts \cite{codabux2021technical}. Although as claimed by the authors \cite{codabux2021technical}, it might represent the comparative distribution of different types of debts in their studied subset of R domain, we need a balanced dataset to develop an unbiased machine learning model. We augmented the text data by replacing adjectives, adverbs, nouns, and verbs with their synonyms to generate different texts with the same meaning \cite{synonym_replace_text_aug_1,synonym_replace_text_aug_2,synonym_replace_text_aug_3}. The synonyms were generated using WordNet \cite{miller1995wordnet}. We did not use SMOTE for data augmentation, since it is not effective for the high dimensional numerical representation of text data \cite{smote_prob_for_text}. The statistics of the final dataset is available at Table \ref{dataset_table_1}.  


%To balance the dataset, we used different scales of augmentation for different types of TD and ensured that each type has a minimum of 100 instances. For example, for the smallest group i.e. Versioning TD, we used a scale of 13 which means 13 new sentences are generated for every Versioning TD sentence\gias{Table \ref{dataset_table_1} shows 12 not 13. Can't we generate the scale as follows. divide the largest original number (i.e., 230) by each smaller one and then use that as a scale for augmentation. For example, code has 113 original sentences. then 230/113 = 2 (rounded), so the scale for code is 2. For versioning 230/8 = 29, so the scale for versioning would be 29}. On the other hand, for the largest group i.e. Documentation TD, we did not generate any new sentence (scale of augmentation was 0). More details are available at Table \ref{dataset_table_1}.



==> threats.tex <==
\section{Threats to Validity}\label{sec:threats}
\it{Internal validity} threats relate to authors' bias 
while conducting the analysis. We mitigated the bias in our machine learning models 
by training, testing, and evaluating them using standard practices. There was no common data between the training and test set. We followed existing literature about TD and discussed among co-authors for listing different types of TD and detecting them.
\it{Construct validity} threats relate to the difficulty in finding
data for our study. Our data collection was exhaustive, as we processed more than 13.5K review comments from 1297 approved packages of two different popular platforms (i.e. rOpenSci, BioConductor).  
\it{External validity} threats relate to the
generalizability of our findings. We mitigated this threat by conducting our study on a large-scale data. We experimented with the peer review documentation of R packages to analyze TD. We used two different platforms and compared our findings with previous work as well. Moreover, the performance of our automated framework that we used for our empirical study was satisfactory. Hence, our findings are as generalized as possible and our finding can be applied to other similar platforms and applications. 
